Dual convolution for the affine group of the real line

The Fourier algebra of the affine group of the real line has a natural identification, as a Banach space, with the space of trace-class operators on $L^2({\mathbb R}^\times, dt/ |t|)$. In this paper we study the "dual convolution product" of trace-class operators that corresponds to pointwise product in the Fourier algebra. Answering a question raised in work of Eymard and Terp, we provide an intrinsic description of this operation which does not rely on the identification with the Fourier algebra, and obtain a similar result for the connected component of this affine group. In both cases we construct explicit derivations on the corresponding Banach algebras, verifying the derivation identity directly without requiring the inverse Fourier transform. We also initiate the study of the analogous Banach algebra structure for trace-class operators on $L^p({\mathbb R}^\times, dt/ |t|)$ for $p\in (1,2)\cup(2,\infty)$.

==> fourier-affine_mac.tex <==


\usepackage{amsmath,amsfonts,amssymb}


% ams math allows smaller fractions in displaymode using \tfrac or larger fractions in textmode using \dfrac
% https://tex.stackexchange.com/questions/46369/smaller-fractions-in-displayed-formulae/46372



%%%%%%%%%%%%%%%%%% YC THEOREM CONVENTIONS
\RequirePackage{amsthm}   %Inbuilt environments for defns etc
%\usepackage{theorem}

\newcounter{pulse}[section]
\numberwithin{pulse}{section}  % all thms, etc set from pulse
\numberwithin{equation}{section}

%Styles for theorems, definitions, remarks

\newcommand{\thf}{\sc} % alias for theorem heading font

%-Theorems
\theoremstyle{plain}
\newtheorem{thm}[pulse]{\thf Theorem}
\newtheorem*{thmstar}{\thf Theorem}
\newtheorem{prop}[pulse]{\thf Proposition}
\newtheorem{lem}[pulse]{\thf Lemma}
\newtheorem{cor}[pulse]{\thf Corollary}
%-Definitions
\theoremstyle{definition}
\newtheorem{dfn}[pulse]{\thf Definition}
\newtheorem{notn}[pulse]{\thf Notation}
\newtheorem{eg}[pulse]{\thf Example}
%-Remarks
\theoremstyle{remark}
\newtheorem{rem}[pulse]{\thf Remark}
\newtheorem*{remstar}{\thf Remark}


%% YC's own hack instead of the enumerate package
\newenvironment{romnum}{%
\begin{enumerate}
\renewcommand{\labelenumi}{{\rm(\roman{enumi})}}
\renewcommand{\theenumi}{{\rm(\roman{enumi})}}
}{\end{enumerate}\ignorespacesafterend}

\newenvironment{alphnum}{%
\begin{enumerate}
\renewcommand{\labelenumi}{{\rm(\alph{enumi})}}
\renewcommand{\theenumi}{{\rm(\alph{enumi})}}
}{\end{enumerate}\ignorespacesafterend}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\newcommand{\twomat}[4]{\left[ \begin{matrix} #1 & #2 \\ #3 & #4 \end{matrix} \right]}
\newcommand{\ptp}{\mathbin{\widehat{\otimes}}}
\newcommand{\tp}{\mathbin{\otimes}}
\newcommand{\abs}[1]{{\vert#1\vert}}
\newcommand{\norm}[1]{{\Vert#1\Vert}}
\newcommand{\ip}[2]{\langle#1, #2\rangle}

\newcommand{\pair}[2]{{\langle#1, #2\rangle}}
% want to try and keep a distinction in the source code between "inner product" and "bilinear pairing"


% for induced representations
\newcommand{\Ind}{\operatorname{Ind}}
% for direct integrals
\newcommand{\dirint}{\int^{\oplus}}

\newcommand{\al}{\alpha}
\newcommand{\lm}{\lambda}
\newcommand{\om}{\omega}
\newcommand{\Om}{\Omega}

\newcommand{\sH}{\mathsf{H}}


\newcommand{\cA}{{\mathcal A}}
\newcommand{\cB}{{\mathcal B}}
\newcommand{\cF}{{\mathcal F}}
\newcommand{\cH}{{\mathcal H}}
\newcommand{\cS}{{\mathcal S}}
\newcommand{\cT}{{\mathcal T}}
\newcommand{\cU}{{\mathcal U}}

\newcommand{\sV}{{\mathsf{V}}}
\newcommand{\sW}{{\mathsf{W}}}

%%\newcommand{\GL}{\operatorname{GL}\nolimits}
\newcommand{\FA}{{\rm A}}
\newcommand{\VN}{{\rm VN}}
\newcommand{\GL}{{\rm GL}}
%\newcommand{\Aff}{\operatorname{Aff}}
\newcommand{\sgn}{{\rm sign}}

\newcommand{\sHbar}{\overline{\sH}}



%%%%%%%%%%%%%%%%%%%

% YC aliases (force of habit)
\newcommand{\Cplx}{{\mathbb C}}
\newcommand{\Real}{{\mathbb R}}

\newcommand{\Rx}{{\Real^\times}}
\newcommand{\Rxpos}{{\Real^\times_1}}
\newcommand{\affR}{{\Real\rtimes\Rx}}
\newcommand{\affRpos}{{\Real\rtimes\Rxpos}}

\newcommand{\Bdd}{{\mathcal B}}

%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\tilbox}{\widetilde{\boxtimes}}

% following is for explaining steps in a chain of aligned equations
\newcommand{\expo}[1]{\text{\small\textsf{[#1]}}}

\newcommand{\defeq}{\mathbin{:=}}

% Macro version of MG's notation
\newcommand{\ONE}{\operatorname{I}}
\newcommand{\TWO}{\operatorname{II}}
\newcommand{\THREE}{\operatorname{III}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\sameforeta}{\ensuremath{\underline{\textsf{repeat for } {\boldsymbol{\eta}}}}}
\newcommand{\REPEAT}[1]{\ensuremath{\underline{#1}\tp \sameforeta}}


